Balancing Confidentiality and Transparency for Blockchain-based Process-Aware Information Systems

Blockchain enables novel, trustworthy Process-Aware Information Systems (PAISs) by enforcing the security, robustness, and traceability of operations. In particular, transparency ensures that all information exchanges are openly accessible, fostering trust within the system. Although this is a desirable property to enable notarization and auditing activities, it also represents a limitation for such cases where confidentiality is a requirement since interactions involve sensitive data. Current solutions rely on obfuscation techniques or private infrastructures, hindering the enforcement capabilities of smart contracts and the public verifiability of transactions. Against this background, we propose CONFETTY, an architecture for blockchain-based PAISs to preserve confidentiality and transparency. Smart contracts enact, enforce and store public interactions, while attribute-based encryption techniques are adopted to specify access grants to confidential information. We assess the security of our solution through a systematic threat model analysis and evaluate its practical feasibility by gauging the performance of our implemented prototype in different scenarios from the literature.

==> addon/commands-for-inline-referenceable-objects-with-counter.tex <==
%%%% A command for inline requirements. This one alters the counter from arabic to arabic with an "R" prefix, boldface
%%%% ----------------------------------------------------------------
\newcounter{req}
% When defining a new counter, say ``req'', then command ``\thereq'' is generated automatically. Hence the need for a ``\renewcommand''
\renewcommand{\thereq}{R\arabic{req}}
\newcommand\aReq[0]{%
	\refstepcounter{req}%
	\textbf{\thereq}}
% For the references with the cleveref package
\RequirePackage{cleveref}
\crefname{req}{Req.}{Reqs.}
\Crefname{req}{Requirement}{Requirements}
%%%% Usage example:
%%%%   Our work firstly pursues the objective of preserving \Req\label{req:secrecy} in process data treatment.
%%%%   [..]
%%%%   Therefore, our approach aims to yield \cref{req:secrecy}






%%%% A command for inline requirement list. This one alters the counter from arabic to arabic with an "R" prefix, boldface
%%%% ----------------------------------------------------------------
\RequirePackage[inline]{enumitem}
%
\def\requiprefix{R}
\def\requinum{\requiprefix\arabic*}
% https://tex.stackexchange.com/questions/410585/cleveref-format-for-enumerate    
\newlist{requiilist}{enumerate*}{1}  % create a new enumerate-like environment
\setlist[requiilist,1]{label={(\textbf{\requinum})},itemjoin={},before={},ref=\requinum}
% For the references with the cleveref package
\RequirePackage{cleveref}
\crefname{requiilisti}{requirement}{requirements} % requiilist*i* to indicate level 1 (automatically assigned)
\Crefname{requiilisti}{Requirement}{Requirements}
%%%% Usage example:
%%%%   \begin{requiilist}
%%%%   	\item Monitor parties must [...] \label{req:trustworthiness}
%%%%    [..]
%%%%   \end{requiilist}
%%%%   [..]
%%%%   articles for each of \cref{req:trustworthiness,req:noleakage,req:nopeeking,req:operativeness}
%%%%   [..]
%%%%   \ref{req:trustworthiness} 
%%%%   Therefore, our approach aims to yield \cref{obj:secrecy}
